Reduction in X does not agree with Intersection and Union Types (Extended abstract)

This paper defines intersection and union type assignment for the calculus X, a substitution free language that enjoys the Curry-Howard correspondence with respect to Gentzen's sequent calculus for classical logic. We show that this notion is closed for subject-expansion, and show that it needs to be restricted to satisfy subject-reduction as well, making it unsuitable to define a semantics.

==> macros.tex <==
%{

\def \Bf#1{\mbox{\bf #1}}
\def \Rm#1{\mbox{\rm #1}}
\def \It#1{\mbox{\sl #1}}
\def \Sf#1{\mbox{\small \sf #1}}
\def \Sfb#1{\mbox {\sfb #1}}
\def \Sc#1{\mbox{\sc #1}}

\makeatletter
\def\ifnextchar{\@ifnextchar}
%\setbox144=\hbox{\leavevmode\raise0\point\hbox{{\rm [\kern-1.5\point[}}}
%\setbox145=\hbox{\raise0\point\hbox{{\rm ]\kern-1.5\point]}}}
\setbox144=\hbox{\leavevmode\raise1\point\hbox{${\lceil}\kern-3\point{\lceil}$}}
\setbox145=\hbox{\raise1\point\hbox{${\rfloor}\kern-3\point{\rfloor}$}}
\setbox146=\hbox{$\vdash$\kern-3.5\point\raise5.5\point\hbox{\scriptsize r}}
\setbox147=\hbox{$\vdash$\kern-3.5\point\raise5.5\point\hbox{\scriptsize $\perp$}}
\setbox148=\hbox{\kern-1\point {\footnotesize ${-}\kern-5.5\point \omega \kern -5.5\point{-}$\kern-0pt}}
\setbox149=\hbox{{\footnotesize $\cap$}}

\def \sqsubset{\psset{linewidth=0.4\point}
	\psline{c-c}(1\point,0.4\point)(1\point,6\point)
	\psline{c-c}(1\point,6\point)(7.5\point,6\point)
	\psline{c-c}(1\point,0.4\point)(7.5\point,0.4\point)
}
\def \boxtilde{\sqsubset\kern.1\point\raise-4.5\point\hbox{$\equr$}}

\def \lsem	{\Rm{[\kern-.11em[}}
\def \rsem	{\Rm{]\kern-.11em]}}
\def \PFV#1{\It{pfv}(#1)}%{\It {P\kern-.1em F\kern-.03em V}\,(#1)}
\def \FV#1{\textsl {fv}\psk(#1)}%{\textsl {FV}\,(#1)}
\def \BV#1{\textsl {bv}\psk(#1)}%{\textsl {BV}\,(#1)}
\def \after 	{\mbox{\hspace*{.5\point}$\circ$}\hspace*{1\point}}
\def \Id	{\textsl {id}}

\def \tab {\hspace*{1cm}}
% \def \tab {\hfill}
 \def \n {\underline{n}}
 \def \m {\underline{m}}
 \def \k {\underline{k}}
 \def \p {\underline{p}}
 \def \intn {{\cap}_{\n}}
 \def \intm {\cap_{\m}}

\def \QED {\kern3mm%\hfill
\hbox{\rule{5.5\point}{5.5\point}\hspace*{.5\leftmarginii}}}

\def \dblambda	{\psset{unit=1\point,linewidth=.75\point}%
\psline{-}(.9,0.45)(2,.8)%
\psline{-}(1.75,.55)(2.1,2.1)%
\lambda \kern-.5em\raise.15em\hbox{$\lambda$}\,}

\def \cormargin {\advance\@enumdepth}
\def \martab	{\ifnum \@enumdepth>1%
	\else{\ifnum\@enumdepth>0\else \hspace*{\leftmarginiii}%
	\fi}\hspace*{\leftmarginiv}\fi \hspace*{\leftmarginv}}

\def\Array{%\vspace*{-\baselineskip}
\[\begin{array}{rcll}
\leftmargin -\@totalleftmargin
}
\def\endArray{\vspace*{-2\point}\end{array}\]}

%\newcommand{\rootp}{{\scriptstyle \Lambda}}
\newcommand{\Rhd}{\triangleright}
\newcommand{\Lhd}{\triangleleft}

\def \lineitem {\vspace*{6\point} \noindent\hbox to \leftmarginii{\hfill --\hspace*{\labelsep}}}
\def \bulletitem {\par\vspace*{2\point}\noindent\hbox to \leftmarginii{\hfill {\small $\bullet$}\hspace*{\labelsep}}}

\def \ssrm{\scriptsize \rm}
\def \tsrm{\tiny \rm}

\def \scbf#1{\mbox{\scriptsize \bf #1}}
\def \scrm#1{\mbox{\scriptsize \rm #1}}
\def \scit#1{\mbox{\scriptsize \it #1}}
\def \sctt#1{\mbox{\scriptsize \tt #1}}
\def \scsf#1{\mbox{\scriptsize \sf #1}}
\def \scsc#1{\mbox{\scriptsize \sc #1}}
\def \scsl#1{\mbox{\scriptsize \sl #1}}

\def \cmrit	{\small}

\def \alltv	{\mbox	{$\forall$}}

% \def \prB#1{\mbox	{$\Pi\{#1\}$}}

\def \dots	{\mbox	{$\cdots$}}

\def \adjustmath	{\kern-2\point}

% commands with parameters
\newskip \emskip \emskip0.3\point
% \def \It#1{\kern-\emskip \mbox{\it #1}\kern\emskip}
\def \Em#1{\kern-\emskip{\it #1}\kern\emskip}

\def \Vars#1{\textsl {Var}\,(#1)}
\def \FVar {\makebox {$\Phi$}}
\def \BVar {\makebox {${\cal A}$}}

\def \TypeVar {\makebox {$\cal V$}}
\def \Sorts {\makebox {$\cal S$}}

% small white space
\def \psk	{\hspace*{0.5pt}}
\def \sk	{\hspace*{1pt}}
\def \skp	{\hspace*{1.5pt}}
\def \Skip	{\hspace*{2pt}}
\def \fsk {\hspace*{0.04em}}
\def \lsk	{\hspace*{3\point}}
\def \msk	{\hspace*{2\point}}
\def \ssk	{\hspace*{1.25\point}}
\def \bs	{\mbox	{$\!$}}
\def \emptyline	{\vskip 10\point plus 5\point minus 4\point \noindent}
\def \stab	{\hspace*{0.5\leftmarginii}}
% \def \tab	{\hspace*{\leftmarginii}}
\def \dquad {\quad \quad}
\def \tquad {\quad \quad \quad}
\def \qquad {\quad \quad \quad \quad}

% seq relations
\def \beq	{\mathop{\geq}}
\def \beqe	{\mathop{\geq_{\scsc{e}}}}
\def \seq	{\mathop{\leq}}
\def \seqs	{\mathop{\leq_{\scsc{s}}}}
\def \seqe	{\mathop{\leq_{\scsc{e}}}}
\def \beqe	{\mathop{{\beq\kern-2pt_{\scsc{e}}}}}
\def \seqOne	{\mathop{ \seqr_{\scit {1}} }}
\def \seqTwo	{\mathop{\seqr_{\scit {2}}}}
\def \seqC	{\mathop{ \seqr_{\scit {C}} }}
\def \seqn	{{\,{\leq}\,}}
\def \equr	{{\sim}}
\def \equ	{\mathop{ \equr }}
\def \equTwo	{\mathop{ \equr_{\scit {2}} }}
\def \equs	{\mathop{{\sim}_{\scsc{s}}}}
\def \eque	{\mathop{{\sim}_{\scsc{e}}}}

% logical relations
\def \Times	{\mbox	{$~\times\ $}}
\def \And	{~\&\ }
\def \Or	{~$\vee$ }
\def \If	{\mathrel{\Ifr}} 
\def \Ifr	{\Leftarrow}
\def \Iffs	{\mbox	{$\Leftarrow\kern-6\point\Rightarrow$}}
\def \Iffr	{\Iffs}
\def \Iff	{\mathrel{\Leftarrow\kern-6pt\Rightarrow}}
\def \Exists {\exists\skp}
\def \Forall {\forall\skp}
% \def \Then	{\Skip\,\Thenr\,\Skip}
\def \Thenr	{{\Rightarrow}}
\def \Thenbr(#1){\mathrel{\Thenr~(#1)}}
\def \Then{\@ifnextchar({\Thenbr}{\mathrel{\Rightarrow}}}
\def \Implyr	{{\Rightarrow}}
\def \Implyone#1{\Skip\,\Implyr\,(#1)\,\Skip}
\def \Imply{\@ifnextchar{\bgroup}{\Implyone}{\Skip\,\Implyr\,\Skip}}
\def \IH{\textit{IH}}

% set operations
\def \bar	{\mathop{ \clbar }}
\def \clbar	{\mbox	{$\mid$}}
\def \Empty	{\emptyset}%{\mbox	{$\emptyset$}}
\def \notele	{\mathbin{\not\in}}
\def \ele	{\mathbin{\in}}
\def \Subseteq	{\subseteq}%{\mbox	{$\lsk\subseteq\lsk$}}
\def \Supseteq	{\supseteq}%{\mbox	{$\lsk\supseteq\lsk$}}
\def \Except	{\setminus}%{\mbox	{$\setminus$}}
\def \Union	{\bigcup}
\def \union	{\mathop{\cup}}
\def \Lub	{\bigsqcup}

% indices between values
\def \jotm	{\mbox	{$1{\,\leq\,} j{\,\leq\,}m$}}
\def \iotm	{\mbox	{$1{\,\leq\,} i{\,\leq\,}m$}}
\def \iotn	{\mbox	{$1{\,\leq\,} i{\,\leq\,}n$}}
%\def \ijotn	{\mbox	{$1{\,\leq\,} i_j{\,\leq\,}n$}}
\def \ijotn	{i_j \ele \n}
\def \iotnmo	{\mbox	{${\,\leq\,} i{\,\leq\,}n{-}1$}}
\def \iztn	{\mbox	{$0{\,\leq\,} i{\,\leq\,}n$}}
\def \jotn	{\mbox	{$1{\,\leq\,} j{\,\leq\,}n$}}
\def \jiotm	{\mbox	{$1{\,\leq\,} j_i{\,\leq\,}m$}}
\def \injotn	{\mbox	{$1{\,\leq\,}i{\,\not\hspace*{.5\point}=\,}j{\,\leq\,}n$}}
\def \lotkj {l \ele \underline{k_j}}

% relations
\def \notid	{\not=}%{\mbox	{\mathop{$\not\hspace*{.5\point}=$}}}
\def \same	{\mbox	{\mathop{$\equiv$}}}
\def \notsame	{\mathop{{\not\equiv}}}
\def \after	{\mbox	{$\circ$\hspace*{0.5\point}}}
\def \about	{\mbox	{$\ssk\approx\ssk$}}
\def \con	{\mbox	{$\ssk\ast\ssk$}}

% enumerations of types
\def \aotn	{\mbox	{$\alpha_1, \ldots, \alpha_n$}}
\def \motn	{\mbox	{$\mu_1, \ldots, \mu_n$}}
\def \sotm	{\mbox	{$\sigma_1, \ldots, \sigma_m$}}
\def \sotn	{\mbox	{$\sigma_1, \ldots, \sigma_n$}}
\def \sotnpoa	{\mbox	{$\sigma'_1, \ldots, \sigma'_{n+1}$}}
\def \totn	{\mbox	{$\tau_1, \ldots, \tau_n$}}
\def \totm	{\mbox	{$\tau_1, \ldots, \tau_m$}}

% type operators
\def \inter	{{\copy149}}
% \def \inter	{{\cap}}
\def \Inter	{\mbox	{\,$\cap$\,}}
\def \arrow	{{\rightarrow}}
\def \arr	{{\rightarrow}}
\def \vfi	{\varphi}

% often used types
\def \aAb	{\alpha{\rightarrow}\beta}
\def \aIb	{\alpha \inter \beta}
\def \dAm	{\delta{\arr}\mu}
\def \rAm	{\rho{\arr}\mu}
\def \gAd	{\gamma{\arr}\delta}
\def \gAdIn	{(\gamma_1{\arr}\delta_1) \Inter \dots \Inter (\gamma_n{\arr}\delta_n)}
\def \sIt	{\sigma \inter \tau}
\def \sAt	{\sigma{\arr}\tau}
\def \rAm	{\rho{\arr}\mu}
\def \rAs	{\rho{\arr}\sigma}
\def \rAt	{\rho{\arr}\tau}
\def \tAs	{\tau{\arr}\sigma}
	
% tupels

% arrow types
\def \goAgnAga {\gamma'_1{\arrow}{\dots}{\arrow}\gamma'_n{\arrow} \gamma'}
\def \goAgnAg {\gamma_1{\arrow}{\dots}{\arrow}\gamma_n{\arrow} \gamma}
\def \moAmnAm {\mu_1{\arrow}{\dots}{\arrow}\mu_n{\arrow} \mu}
\def \soAsnAs {\sigma_1{\arrow}{\dots}{\arrow}\sigma_n{\arrow} \sigma}
\def \soAsmAs {\sigma_1{\arrow}{\dots}{\arrow}\sigma_m{\arrow} \sigma}
\def \soAsnAf {\sigma_1{\arrow}{\dots}{\arrow}\sigma_n{\arrow} \varphi}
\def \soAsnAs {\sigma_1{\arrow}{\dots}{\arrow}\sigma_n{\arrow} \sigma}
\def \stAsnAs {\sigma_2{\arrow}{\dots}{\arrow}\sigma_n{\arrow} \sigma}
\def \soAsnAt {\sigma_1{\arrow}{\dots}{\arrow}\sigma_n{\arrow} \tau}
\def \toAtnAt {\tau_1{\rightarrow}{\dots}{\rightarrow}\tau_n{\rightarrow} \tau}

% bases
\def \Bases	{\mbox	{$\cal B$}}
\def \Botn	{\mbox	{$B_1, \ldots, B_n$}}
\def \Botna	{\mbox	{$B'_1, \ldots, B'_n$}}
\def \Botm	{\mbox	{$B_1, \ldots, B_m$}}
\def \Botma	{\mbox	{$B'_1, \ldots, B'_m$}}
\def \PoPm	{\mbox	{$P_1, \ldots, P_m$}}
\def \PoPn	{\mbox	{$P_1, \ldots, P_n$}}

\def \ppd{\textsl {pp}}
\def \ppone(#1){\ppd\,(#1)}
\def \pp{\@ifnextchar({\ppone}{\ppd}}

\def \Pe	{\mbox	{${\cal P}$}}

\def \noomega	{\copy148}

\def\BCD{\textsc{bcd}}
\def\BCDscript{\mbox{\scsc{bcd}}}
\def\CDscript{\mbox{\scsc{cd}}}
\def\Cscript{\mbox{\scsc{c}}}
\def\CDVscript{\mbox{\scsc{cdv}}}
% turnstyles
\def \supbot {\kern-3\point\raise5\point\hbox{{\tiny $\perp$}}\kern-.5\point}
\def \subbot {\kern-3\point\raise-2\point\hbox{{\tiny $\perp$}}\kern-.5\point}
\def \Turn	{\mathbin{\vdash}}
\def \TurnBCD	{\mathbin{{\vdash}\kern-2pt_{\BCDscript}}}
%\def \TurnBot	{\mathbin{{\vdash}\supbot}}
\def \TurnBot	{\mathbin{{\vdash}\subbot}}
\def \TurnBotStrict	{\mathbin{{\vdash}\supbot\kern-2\point_{\scit {S}}}}
\def \TurnBotR	{\mathbin{{\vdash}\supbot\kern-2\point_{\scit {R}}}}
\def \TurnBotER	{\mathbin{{\vdash}\supbot\kern-2\point_{\scit {R}}}}
%\def \TurnC {\mathbin{{\vdash}\kern-2\point_{\scrm {C}}}}
\def \TurnC	{\mathbin{{\vdash}\kern-2pt_{\Cscript}}}
\def \TurnCD	{\mathbin{{\vdash}\kern-2pt_{\CDscript}}}
\def \TurnCDV	{\mathbin{{\vdash}\kern-2pt_{\CDVscript}}}
\def \TurnCh {\mathbin{{\vdash}\kern-2\point_{\scsc {Ch}}\kern-2\point}}
\def \TurnE {\mathbin{{\vdash}\kern-2\point_{\scsc{e}}}}
\def \TurnEnv {\mathbin{{\vdash}\kern-2\point_{{\cal E}}}}
\def \TurnEBot	{\mathbin{{\vdash}\supbot\kern-3\point_{\cal E}}}
\def \TurnECL	{\mathbin{{\vdash}\kern-1\point_{{\cal E}_{\mbox{\tsrm CL}}}}}
\def \TurnEw	{\mathbin{{\vdash}\kern-1\point_{{\cal E}}^{\noomega}}}
\def \TurnI {\mathbin{{\vdash}\kern-2\point_{\mbox{\tiny$\cap$}}}}
\def \TurnInt {\mathbin{{\vdash}\kern-2\point_{\cap}}}
\def \TurnLambda	{\TurnLambdar}
\def \TurnLambdar	{\mathbin{{\vdash}\kern-1\point_{\lambda\cap}}}
\def \TurnMyc {\mathbin{{\vdash}\kern-2\point_{\scsc {Myc}}\kern-2\point}}
\def \TurnML {\mathbin{{\vdash}\kern-2\point_{\scsc {ml}}\kern-2\point}}
\def \TurnQ {\mathbin{{\vdash}\kern-2\point_{\forall}}}
\def \TurnR	{\mathbin{{\vdash}\kern-2\point_{\scsc {r}}}}
\def \TurnRel	{\mathbin{{\vdash}\kern-2\point_{\scsc {r}}}}
\def \TurnSE	{\mathbin{{\vdash}_\leq}}
\def \Turnsn	{\mathbin{{\vdash}\kern-3\point_{\noomega}}}
\def \TurnStrict	{\mathbin{{\vdash}\kern-2\point_{\scsc {s}}}}
\def \TurnTwoE	{\mathbin{{\vdash_{\cal E}^{\scit {2}}}}}
\def \Turnw	{\mathbin{{\vdash}^{\noomega}}}

 \def \TurnEr	{\lsk\copy146\kern-1\point_{\cal E}\lsk}

 \newcount\derW
 \newcount\hderW
 \newcount\botW
 \newcount\hbotW
 \newcount\topW
 \newcount\htopW
 \newcount\boxshift


\def \rsk {\vspace*{5mm}}
\def	\Deriv#1{\langle #1\rangle}

\def \Stat#1#2{{\termcolour #1}\sk{:}\ssk{\typecolour #2}}
\def \Modthree#1#2#3{#1 \model \Stat{#2}{#3}}
\def \Mod#1#2{\@ifnextchar{\bgroup}{\Modthree{#1}{#2}}{#1 \model {#2}}}
\def \Modsthree#1#2#3{#1 \dTusimple \Stat{#2}{#3}}
\def \Mods#1#2{\@ifnextchar{\bgroup}{\Modsthree{#1}{#2}}{#1 \dTusimple {#2}}}
\def \DerBCD#1#2#3{#1\TurnBCD \Stat{#2}{#3}}
\def \DerE#1#2#3{#1 \Turne \Stat{#2}{#3}}
\def \Der#1#2#3{{\typecolour #1} \Turn \Stat{#2}{#3}}
\def \der#1|-#2 : #3 {{\typecolour #1} \Turn \Stat{#2}{#3} }
\def \derBCD#1|-#2 : #3 {{\typecolour #1}\TurnBCD \Stat{#2}{#3} }
\def \derC#1|-#2 : #3 {{\typecolour #1} \TurnC \Stat{#2}{#3} }
\def \derCD#1|-#2 : #3 {{\typecolour #1} \TurnCD \Stat{#2}{#3} }
\def \derCDV#1|-#2 : #3 {{\typecolour #1} \TurnCDV \Stat{#2}{#3} }
\def \derE#1|-#2 : #3 {{\typecolour #1} \TurnE \Stat{#2}{#3} }
\def \derI#1|-#2:#3 {#1 \TurnI \Stat{#2}{#3}}
\def \derR#1|-#2 : #3 {{\typecolour #1} \TurnR \Stat{#2}{#3} }
\def \derS#1|-#2 : #3 {{\typecolour #1} \TurnStrict \Stat{#2}{#3} }
\def \derRel#1|-#2 : #3 {{\typecolour #1} \TurnR \Stat{#2}{#3} }
%
\def \DerSE#1#2#3{#1 \TurnSE \Stat{#2}{#3}}
\def \DerBot#1#2#3{#1 \TurnBot \Stat{#2}{#3}}
\def \DerBotE#1#2#3{#1 \TurnBotE \Stat{#2}{#3}}
\def \derBot#1 |- #2 : #3 {{\typecolour #1} \TurnBot \Stat{#2}{#3}}
\def \DerBotR#1#2#3{#1 \TurnBotR \Stat{#2}{#3}}
\def \DerBotER#1#2#3{#1 \TurnBotR \Stat{#2}{#3}}
\def \DerC#1#2#3{#1 \TurnC \Stat{#2}{#3}}
\def \DerCh#1#2#3{#1 \TurnCh \Stat{#2}{#3}}
%\def \DerE#1#2#3{#1 \TurnE \Stat{#2}{#3}}
\def \DerRel#1#2#3{#1 \TurnR \Stat{#2}{#3}}
\def \DerECL#1#2#3{#1 \TurnECL \Stat{#2}{#3}}
\def \DerML#1#2#3{#1 \TurnML \Stat{#2}{#3}}
\def \DerMyc#1#2#3{#1 \TurnMyc \Stat{#2}{#3}}
\def \DerInt#1#2#3{#1 \TurnInt \Stat{#2}{#3}}
\def \DerStrict#1#2#3{#1 \TurnStrict \Stat{#2}{#3}}
\def \Dersn#1#2#3{#1 \Turnsn \Stat{#2}{#3}}
\def \DerQ#1#2#3{#1 \TurnQ \Stat{#2}{#3}}
\def \DerR#1#2#3{#1 \TurnTwoE \Stat{#2}{#3}}
\def \Derw#1#2#3{#1 \Turnw 	\Stat{#2}{#3}}

% reduction symbols
\def \bredr	{\mbox	{$\rightarrow_{\beta}$}}
\def \eredr	{\mbox	{$\rightarrow_{\eta}$}}
\def \eqbr	{{=_{\beta}}}
\def \eqb	{\mathrel{=_{\beta}}}
\def \eqRs	{=_{\mbox{\scbf R}}}
\def \eqR	{{\ \eqRs}\ }
\def \noteqvR	{{\ \not\kern-3\point\eqvRs}\ }
\def \eqvRs	{{\approx_{\mbox{\scbf R}}}}
\def \eqvR	{\mathop{\eqvRs}}
\def \eqvRhnfs	{{\approx_{\mbox{\scbf R}}^{\scit {hnf}}}}
\def \eqvRhnf	{\mathop{\eqvRhnfs}}
\def \bred	{\mathop{\bredr}}
\def \ered	{\mathop{\eredr}}
\def \dbredr	{\arrow \kern-.7em\bredr}
\def \dbred	{\mathop{\dbredr}}

\def \redir {,}%{\,{\triangleright}\,}
\def \redbot	{\mathop{\mbox{$\rightarrow_{\beta\bottom}$}}}
\def \etared	{\mathrel{\arrow_{\eta}}}
\def \reduc	{\mathrel{\Yellow \arrow}}
\def \redplus	{\mbox {\mathop{$\arrow^+$}}}
\def \redpluss	{\mbox	{$\arrow^*$}}
\def \redr	{\mathop{\arrow_{\mbox{\scbf r}}}}
\def \dred	{\mathrel{\rightarrow^*}}
\def \lored	{\mathop{\arrow_{\mbox{\scsl {lor}}}}}
\def \Lor(#1){\mbox{{\sl lor}$(#1)$}}

\def \redC	{\mbox {\mathop{\redCs}}}
\def \redCs	{$\rightarrow_C$}
\def \redp	{\mbox{\mathop{$\rightarrow^+$}}}

\def \redRps	{\mbox	{$\rightarrow^+_{\mbox{\scbf R}}$}}
\def \dredR	{{\ \dredRs}\ }
\def \dredRs	{\rightarrow^*_{\mbox{\scbf R}}}

\def\RtauB	{\R^{\tau}_B}
\def\redR	{\mathrel{\arrow_{\mbox{\scbf R}}}}
\def\redb	{\mathrel{\arrow_\beta}}
\def\redRb	{\red}

\def \derred	{\mathrel{{\rightarrow}_{\cal D}}}
\def \dderred	{\mathrel{\derred^*}}


% special symbols
\def \TRSbeta	{\Sc{trs}\,{+}\,\beta}

\def \refer#1{(\It {#1})\hspace{5\point}}
\def \Refer#1{\hfill{(\Em {#1})}\hspace*{.5\leftmarginii}}
\def \NLRefer#1{\\\hspace*{\leftmarginii}\hfill{(\Em {#1})}\hspace*{.5\leftmarginii}}

\def \pow	{\mbox	{$\wp$}}
\def \bottom	{{\perp}}
\def \tbot	{t_{{\perp}}}

%
% trs macros
%
\def \trs	{\mbox	{$(\Sigma, \Rules)$}}
\def \ctrs	{\mbox	{$(\Sigma, \Rules)$}}
\def \CTRS	{\mbox{{\small {\it C\kern-3\point u}\kern-1\point{TRS}}}}
\def \atrs	{\Aps\kern-1\point{TRS}}
\def \Terms	{\mbox	{$\textsl {T}({\cal F}\kern-.3em, {\cal X})$}}

% special symbols
\def \FuncAp	{\mbox	{${\cal F}\,{\cup}\,\{Ap\}$}}
\def \Envone#1{{\cal E}\psk(#1)}
\def \Env{\@ifnextchar{\bgroup}{\Envone}{{\cal E}}}
\def \Enva	{\mbox	{$\Env'$}}
\def \EnvCL	{\Env_{\mbox{\scsc{cl}}}}
\def \Newenv#1#2{\Env\,[#1\,{:=}\,#2]}%{\Env\psk[#1\,{:=}\,#2]}

\def \arity#1{\mbox	{\textsl {arity}\psk $(#1)$}}

\def \rhd {\mbox {\rule[-.03em]{.04em}{0.55em}\kern-.125em{$>$}}}
\def \Subterm	{\mbox	{\raise-.5\point\hbox{\rule{.6\point}{6.5\point}}\kern-1\point$>$}}
\def \SubtermChnf	{\mbox	{\, $\rhd_{\mbox {\scit Chnf}}$}}
\def \Subtermmul	{\mbox	{\, $\rhd_{\mbox {\scit mul}}$}}
\def \TSubRed	{\mbox	{(\botreds \union \Subterm)$_{\mbox {\scit mul}}$}}
\def \SubRed	{\mbox	{(\redRs \union \Subterm)$_{\mbox {\scit mul}}$}}

\def \Encomr	{\leavevmode{\setbox150=\hbox{\Subterm}
\setbox151=\hbox {\begin{minipage}{10pt}{\LARGE $\cdot$}\end {minipage}}%
\hbox{\copy150\kern-\wd150\raise-0.05\ht150\box151}}}

\def \Encom	{\mbox	{\mathop{\Encomr}}}

\def \Comps {\textsl{Comp}}
\def \CompOne#1{\mbox{$\Comps\skp(#1)$}}
\def \Comp{\@ifnextchar{\bgroup}{\CompOne}{\Comps}}

% \def \Comp#1{\mbox	{$\textsl {Comp}\,(#1)$}}


% approximants
\def \AppNF	{{\termcolour \cal A}}
\def \appA#1{A\ele {\cal A}(#1)}
\def \AppSem#1{{\cal A}\sk(#1)}
\def \SetAppOne(#1){{\cal A}(#1)}
\def \SetApp{\@ifnextchar({\SetAppOne}{{\cal A}}}
\def \SetAppCS#1{\mbox	{$\AppCS\psk(#1)$}}
\def \SetAppCL#1{\mbox	{$\AppCL\psk(#1)$}}
\def \APP	{\mbox {${\cal A}$}}
\def \AppCS	{\mbox {${\cal A}_{\cal C}$}}
\def \AppCL	{\mbox {${\cal A}_{\mbox{\scsc cl}}$}}
%\def \Approx#1{\mbox	{${\cal A}\textsl{ppr}\,(#1)$}}
\def \Approx#1{\textsl{Appr}\,(#1)}
\def \eappr#1{\Exists {\termcolour A}\ele \AppSem{#1}}
\def \ExAppr#1#2#3{\eappr{{\termcolour #2}} \Pred[\Der{#1}{A}{#3}]}
\def \ExApprE#1#2#3{\eappr{{\termcolour #2}} \Pred[\derE {#1} |- {A} : {#3} ]}
\def \Appr#1#2#3{\eappr{#2}\ \Pred[\Der{#1}{A}{#3}]}
\def \Appre#1#2#3{\eappr{#2}\ \Pred[\derE {#1} |- {A} : {#3} ] }
\def \Apprs#1#2#3{\eappr{#2}\ \Pred[\Ders{#1}{A}{#3}]}

\def \Appra#1#2#3{\Exists $A'\ele {\cal A}\,(#2)$ $[#1$\TurnE $A'{:}#3]$}

\def \appr#1#2#3{\eappr	{\mbox	{$#2$}} [$#1$\TurnE $a{:}#3$]}

\def \DirApp#1{\mbox	{$\cal D$\kern-4\point\lower1\point\hbox{${\cal A}$}\,$(#1)$}}
\def \DirAppSet	{{\cal	D}\kern-4\point\lower1\point\hbox{${\cal A}$}}
\def \compat#1#2{\mbox	{$#1\,{\uparrow}\,#2$}}
\def \Notuparrow{\kern2\point\hbox{\footnotesize /}\kern-7.5\point\uparrow\kern-1\point}
\def \notcompat#1#2{\mbox	{$#1\Notuparrow#2$}}



% Terms and combinators
\def \TSKI	{\mbox {$\textsl {T}\kern-2\point_{{\rm CCL}}$}}
\def \SKIterms	{\mbox {$\textsl {T}({\{S,S_2,S_1,S_0,K,K_1,K_0,I,I_0\}, {\cal X}})$}}
\def \NCTerms	{\mbox {$\textsl {T}\kern-2\point_{\scit {NC}}({\cal C\kern-.1em,X})$}}
\def \CTerms	{\textsl {T}({\cal C\kern-.1em, X})}
\def \Terms	{\mbox {$\textsl {T}({\cal F}\kern-.3em, {\cal X})$}}
\def \CTermsBot	{\textsl {T}({\cal C\kern-.1em, X}\kern-.2em,\kern-.1em{\perp})}
\def \TermsBot	{\hbox{$\Em {T}({\cal F}\kern-.3em,{\cal X}\kern-.2em,\kern-.1em{\perp})$}}

\def \Const	{\mbox {${\cal C}$}}
\def \Func	{\mbox	{${\cal F}$}}
\def \vars	{\mbox {${\cal X}$}}
\def \cs	{$(\Sigma,\Rules)$}
\def \FPL	{\Sc{fpl}}
\def \ITD	{\Sc{itd}}
\def \TRS	{\Sc{trs}}
\def \Rules	{\Bf{R}}
\def \ML	{\Sc{ml}}
\def \calR	{{\cal R}}
\def \calS	{{\cal S}}
\def \calI	{{\cal I}}

\def \LCvars {{\cal V}}
\def \comb	{{\cal C}}
\def \CTerms {\Types(\comb\kern-1\point,\LCvars)}
\def \CSpair	{\Pair{\comb,\LCvars}}
\def \CS	{\Sc{cs}}
\def \CL	{\Sc{cl}}
\def \TCL {\Types_{\mbox{\scsc{cl}}}}
\def \CLTerms	{\Types(\{\combS,\combK,\combI\},\LCvars)}
\def \TurFix {(\lambda xy.y(xxy))(\lambda xy.y(xxy))}
\def \CurFix {\lambda {f}.(\lambda x.{f}(xx))(\lambda x.{f}(xx))}
\def \LS {\lambda xyz.xz(yz)}
\def \LD {\lambda x.xx}
\def \LK {\lambda xy.x}
\def \LI {\lambda x.x}
\def \LE {\lambda xy.xy}
\def \LZ {\lambda xy.y}

\def \combS	{\Bf{S}}
\def \combK	{\Bf{K}}
\def \combI	{\Bf{I}}
\def \combJ	{\Bf{J}}
\def \combE	{\Bf{E}}
\def \combD	{\Bf{D}}
\def \combT	{\Bf{T}}
\def \combW	{\Bf{W}}
\def \combX	{\Bf{X}}
\def \combY	{\Bf{Y}}
\def \combZ	{\Bf{Z}}

\def \cH	{\Sfb{H}}

\def \mypreceq {\psset{unit=1\point,linewidth=0.5\point}
\pscurve{cc-cc}(-2,3)(1,3.5)(3,4.5)(4,5.5)
\pscurve{cc-cc}(-2,3)(1,2.5)(3,1.5)(4,.5)
\pscurve{cc-cc}(-2,1.5)(1,.9)(3,-.25)(4,-1.25)
}

%\pscurve{cc-cc}(-2,3)(1,3.5)(3,4.5)(4,5.5)
%\pscurve{cc-cc}(-2,3)(1,2.5)(3,1.5)(4,.5)
%\pscurve{cc-cc}(-2,2)(1,1.4)(3,.25)(4,-.75)

\def \derseq	{\mathbin{\preceq}}
\def \derbeq	{\mathbin{\succeq}}
\def \Tseq	{~\mathop{\tseqr~}}
\def \tseq	{\mathbin{\sqsubseteq}}
\def \tgeq	{\mathop{\sqsupseteq}}
\def \Join	{\mbox	{\mathop{\Large $\sqcup$}}}
\def \join{\mathbin{\sqcup}}
%\def \dirapp {\mathrel{\boxtilde}}
\def \coveringrel	{\mathbin{{\prec}\kern-0.5em{\prec}}}
\def \subA	{\mathbin{{\subseteq}_{\cal A}}}
\def \dirapp {\mathrel{\sqsubseteq}}
\def \approximant {\mathbin{\boxtilde}}

\def \joinaotn	{a_1\psk \join \dots \psk \join a_n}
\def \jointotn	{t_1\psk \join \dots \psk \join t_n}
\def \jointotm	{t_1\psk \join \dots \psk \join t_m}
\def \joinvotn	{v_1\psk {\sqcup} \dots \psk {\sqcup} v_n}
\def \AojAn	{\join_{n}A_i}
\def \NojNn	{N_1 \psk \join \dots \join \psk N_n}
\def \MojMn	{M_1 \psk \join \dots \join \psk M_n}
\def \MojMm	{M_1 \psk \join \dots \join \psk M_m}
\def \MojMma	{M'_1 \psk \join \dots \join \psk M'_m}
\def \Motn	{M_1, \ldots, M_n}
\def \xMoMn	{xM_1{\dots}M_n}
\def \xMoMm	{xM_1{\dots}M_m}
\def \xMoMmN	{xM_1{\dots}M_mN}
\def \xAoAn	{xA_1{\dots}A_n}
\def \Ftotn	{F\psk(t_1, \ldots, t_n)}
\def \Fuotn	{F\psk(u_1, \ldots, u_n)}
\def \Ftotm	{F\psk(t_1, \ldots, t_m)}
\def \Fxotn	{F\psk(x_1, \ldots, x_n)}

\def \ap {\app}%{\psk}
\def \app {\cdot}
\def \Ap {\mbox {\it Ap}}

\def \apCaoan	{\mbox {$C{\ap}a_1{\ap}{\dots}{\ap} a_n$}}
\def \apCuoun	{\mbox {$C{\ap}u_1{\ap}{\dots}{\ap} u_n$}}
\def \apCuouna	{\mbox {$C{\ap}u'_1{\ap}{\dots}{\ap} u'_n$}}
\def \apCpotn	{\mbox {$C{\ap}p_1{\ap}{\dots}{\ap} p_n$}}
\def \apCtotn	{\mbox {$C{\ap}t_1{\ap}{\dots}{\ap} t_n$}}
\def \apCxoxi	{\mbox {$C{\ap}x_1{\ap}{\dots}{\ap} x_i$}}
\def \apCxoxn	{\mbox {$C{\ap}x_1{\ap}{\dots}{\ap} x_n$}}

\def \apxuoun	{\mbox {$x{\ap}u_1{\ap}{\dots}{\ap} u_n$}}
\def \apxaoan	{\mbox {$x{\ap}a_1{\ap}{\dots}{\ap} a_n$}}
\def \apxtotn	{\mbox {$x{\ap}t_1{\ap}{\dots}{\ap} t_n$}}
\def \apxtotm	{\mbox {$x{\ap}t_1{\ap}{\dots}{\ap} t_m$}}

\def \aptott	{\mbox	{$t_1{\ap}t_2$}}
\def \aptotn	{\mbox	{$t_1{\ap}\dots{\ap}t_n$}}
\def \aptotta	{\mbox	{$t'_1{\ap}t'_2$}}
\def \aptottda	{\mbox	{$t''_1{\ap}t''_2$}}
\def \apuout	{\mbox	{$u_1{\ap}u_2$}}

\def \D	{{\cal D}}%{\mbox {\rm D}}
\def \dcol {\msk{::}\msk}
\def \Drv#1{\langle #1\rangle}
\def \Dotm {\D_1, \ldots, \D_m}
\def \Dotn {\D_1, \ldots, \D_n}

\newdimen\One
\One1pt

\def \model	{%\hbox to 0pt{$\vdash$}
\mathop{%\setbox150=\hbox{$\vdash$}\hbox{\lsk\lower.2em\copy150\kern-\wd150\raise.2em{\box150}}
\psset{unit=1pt,linewidth=0.45\point}%
\psline{cc-cc}(1,0)(1,7.25)%
\psline{cc-cc}(1,4.55)(5.5,4.55)
\psline{cc-cc}(1,2.8)(5.5,2.8)
\kern6.5\point
}}

\def \dTu	{\mathbin{\model}}
\def \dTusimple {\mathbin{\model\kern-3\point_{\rm s}}}
\def \dTuF	{\mathbin{\model\kern-3\point_{\textsc{\scriptsize f}}}}

\def \mFBCD	{{\cal F}_{\BCDscript}}
\def \mF	{{\cal F}}%{{\cal F}_\cap}
\def \mFs	{{\cal F}_{\scsc s}}
\def \mFe	{{\cal F}_{\scsc e}}

\def \Sem#1{\copy144{#1}\copy145}
\def \SemMxi#1#2{\copy144{#1} \copy145
\setbox153=\hbox{$_{#2}$}
\setbox154=\hbox{\scriptsize $\cal M$}
\ifdim \wd154 > \wd153 {\copy153\kern-\wd153 \hbox{\raise5\point\hbox{\box154}}}
\else {\raise5\point\hbox{\copy154}\kern-\wd154 \box153}
\fi
}
\def \SemM#1{\@ifnextchar{\bgroup}{\SemMxi{#1}}{\SemMxi{#1}{\xi}}}
\def \SemTwoXi#1#2{\Sem{#1}_{#2}}
\def \SemXi#1{\@ifnextchar{\bgroup}{\SemTwoXi{#1}}{\SemTwoXi{#1}{\xi}}}
\def \Semxi#1{\@ifnextchar{\bgroup}{\SemXi{#1}}{\SemXi{#1}{\xi}}}
%\def \Semxi#1{\@ifnextchar{\bgroup}{\SemXi{#1}}{\SemXi{#1}{\xi}}}

\def \Scottl	{\copy144}
\def \Scottr	{\copy145}
\def \Bxi	{\G_{\xi}}
\def \Bxia	{\G_{\xi'}}
\def \ScottrBxi	{\Scottr_{{\xi}_{`G}}}
\def \Scottrxi	{\Scottr_{\xi}}
\def \Setl	{\{\psk} %}{
\def \Setr	{\psk\}}
\def \Set#1{\Setl #1 \Setr} 
\def \Pred[#1]{~[\ssk #1 \ssk]}
\def \SKItoLC#1{\langle #1 \rangle_{\lambda}}
\def \CStoLC#1{\langle #1 \rangle_{\lambda}}
\def \LCtoSKI#1{\copy144 #1 \copy145_{\mbox{\scsc{cl}}}}
\def \LCtoCS#1{\copy144 #1 \copy145_{\cal C}}
\def \Asem#1{\copy144 #1 \copy145^{\cal A}}
\def \AsemCS#1{\copy144 #1 \copy145^{\cal A}_C}
\def \AsemCSf#1{[\kern-1pt[#1]\kern-1pt]^{\cal A}_C}
\def \Fsem#1{\copy144 #1 \copy145^{\cal F}}
\def \FsemE#1{\copy144 #1 \copy145^{\cal F}_{\xi,{\cal E}}}

\def \Totn	{t_1, \ldots, t_n}
\def \Potn	{p_1, \ldots, p_n}
\def \Aptott	{Ap\psk(t_1, t_2)}
\def \FtoTn	{F\psk (t_1, \ldots, t_n)}

% contexts
\def \cont#1{\mbox{\rm C}[\,#1\,]}

% substitution on terms, replacement
\def \R	{\mbox{\rm R}}
\def \Ra	{\mbox	{$\mbox{\rm R}'$}}
\def \Rda	{\mbox	{$\mbox{\rm R}''$}}
\def \Ri#1{\mbox	{$\mbox{R}_{#1}$}}
\def \repl#1{\mbox	{$#1\raise3\point\hbox{\scrm {R}}$}}
\def \replbot#1{\mbox	{$#1^{{\rm R}_\perp}$}}
\def \repla#1{\mbox	{$#1$\raise3\point\hbox{\scrm {R$'$}}}}
\def \replda#1{\mbox	{$#1$\raise3\point\hbox{\scrm {R'}}}}
\def \repli#1#2{\mbox	{$#2$\raise3\point\hbox{$\scrm {R}_{\mbox{\tiny #1}}$}}}
\def \Repl	{\{x_1{\mapsto}t_1, \ldots, x_n{\mapsto}t_n\}}

\def \unifyR	{\mbox	{$\textsl {unify}_{\scrm {R}}$}}
\def \toTqc#1{\mbox	{$\textsl {to}\Types^\forall_{\scit {C}}\,(#1)$}}

\def \fil	{{\uparrow}}
\def \fils	{{\uparrow}_{\scsc{s}}}
\def \file	{{\uparrow}_{\scsc{e}}}
\def \Filters {{\cal F}}
\def \typeint {\upsilon}

\def \dunBa	{\Chain{n, B, \alpha}}

\arraycolsep2.5pt
\def\arraystretch{1.1}

%\def \addcontentsline#1#2#3{}


\def\calR	{{\cal R}}
\def\calS	{{\cal S}}
\def\calI	{{\cal I}}

\def\Ele	{\,\ele\,}

\def \RC {\cal R\kern-1.5\point C}
%\def \REDs {\calR\kern-1.25\point\textsl{e\kern-1\point d}}
\def \REDs {\textsl{Red}}
%\def \REDone#1{ \REDs \, \lceil \psk #1 \psk \rfloor }
\def \REDone#1{ \REDs \,(#1)}
\def \RED{\@ifnextchar{\bgroup}{\REDone}{\REDs}}
%\def \RED#1{\REDs\,(#1)}
\def \Candtwo#1#2{{\RC}^{#1}\,(#2)}
\def \Cand#1{\@ifnextchar{\bgroup}{\Candtwo{#1}}{{\RC}^{#1}}}

\def \Comput#1{\mbox{$\textsl {Comp}\,(#1)$}}
\def \SNbr(#1){\textsl {SN}\,(#1)}
\def \SNone#1{\textsl {SN}\,(#1)}
\def \SNset {{\cal S\kern-1\point N}}
%\def \SNone#1{#1 \ele \SNset}
\def \SN{\@ifnextchar{\bgroup}{\SNone}{\@ifnextchar({\SNbr}{\SNset}}}

\def \Nums	{{\setbox150=\hbox{{\sf I}}\setbox151=\hbox{{\sf N}}%
	\hbox{\copy150\kern-0.35\wd150\box151}}}
\def \Numsub	{{\setbox150=\hbox{{\scsf I}}\setbox151=\hbox{{\scsf N}}%
	\hbox{\copy150\kern-0.35\wd150\box151}}}
\def\smallerN {>_{\Numsub}}
%\def\ggt {>\!\! >}
\def\ggtSN {\gg^{\scsl {SN}}}
\def\ggtSNthree {\gg^{\scsl {SN}}_3}
\def\ggtSNtwo {\gg^{\scsl {SN}}_2}
\def\ggtSNone {\gg^{\scsl {SN}}_1}

\def \OrderCL	{(\smallerN, \Encomr)_{\scit {lex}}}

\def\R{\mbox{\rm R}}

\def \Grid	{\begin {center}
\begin {picture}(30,20)`
\thinlines
\multiput(0,0)(1,0) {31} {\line(0,1) {20}}
\multiput(0,0)(0,1) {21} {\line(1,0) {30}}
\Comment{
\put(-2,1.5) {\makebox(0,0) {0}}
\put(-2,4) {\makebox(0,0) {1}}
\put(-2,6.5) {\makebox(0,0) {2}}
\put(-2,9) {\makebox(0,0) {3}}
\put(-2,11.5) {\makebox(0,0) {4}}
\put(-2,14) {\makebox(0,0) {5}}
\put(-2,16.5) {\makebox(0,0) {6}}
\put(-2,19) {\makebox(0,0) {7}}
\put(1.5,-2) {\makebox(0,0) {0}}
\put(4,-2) {\makebox(0,0) {1}}
\put(6.5,-2) {\makebox(0,0) {2}}
\put(9,-2) {\makebox(0,0) {3}}
\put(11.5,-2) {\makebox(0,0) {4}}
\put(14,-2) {\makebox(0,0) {5}}
\put(16.5,-2) {\makebox(0,0) {6}}
\put(19,-2) {\makebox(0,0) {7}}
\put(21.5,-2) {\makebox(0,0) {8}}
\put(24,-2) {\makebox(0,0) {9}}
\put(26.3,-2) {\makebox(0,0) {10}}
\put(29,-2) {\makebox(0,0) {11}}
}
\end {picture}
\end {center}}

\def \dots	{\cdots}

\def \LC	{\Sc{lc}}
\def \ML	{\Sc{ml}}

\def \ctrs	{(\Sigma,\Rules)}
\def \Terms	{\textsl {T}({\cal F}\kern-.3em, {\cal X})}
\def \TRS	{\Sc{trs}}
\def \arityOne#1{\textsl{arity}\skp(#1)}
\def \arity{\@ifnextchar{\bgroup}{\arityOne}{\textsl{arity}}}
\def \Left {\textsl{left}}
\def \Right {\textsl{right}}
\def \cB	{\Sfb{B}}
\def \cC	{\Sfb{C}}
\def \cD	{\Sfb{D}}
\def \cE	{\Sfb{E}}
\def \cF	{\Sfb{F}}
\def \cG	{\Sfb{G}}
\def \cH	{\Sfb{H}}
\def \cI	{\Sfb{I}}
\def \cK	{\Sfb{K}}
\def \cS	{\Sfb{S}}
\def \cQ	{\Sfb{Q}}
\def \cZ	{\Sfb{Z}}
\def \foldr {\Sf{foldr}}

\def \FEoEn	{\cF\psk(E_1, \ldots, E_n)}
\def \FEoEm	{\cF\psk(E_1, \ldots, E_m)}
\def \Func	{{\cal F}}
\def \Aps	{\Rm{\symbol{64}}\skp}
\def \aps	{\Rm{\symbol{64}}}
\def \Ap	{\mathbin{\hspace*{1pt}}}
\def \ShareSymb {\Sf{share}}
\def \ShareT#1#2#3{\ShareSymb\ap{#1}\ap\Via\ap{#2}\ap\In\ap{#3}}
%\def \ShareT#1#2#3{\ShareSymb \ap \Redir{#2}{#1} \ap \In \ap{#3}}
\def \Share{\@ifnextchar{\bgroup}{\ShareT}{\ShareSymb}}
\def \Let	{\Sf{let}}
\def \In	{\Sf{in}}
\def \Via	{\Sf{via}}
\def \CycleSymb {\Sf{cycle}}
\def \CycleT#1#2{\CycleSymb\ap{\Pair{\,#1\,}}\ap\In\ap{#2}}
\def \Cycle{\@ifnextchar{\bgroup}{\CycleT}{\CycleSymb}}% {\Sf{cyclic}}
\def \Letrec	{\Sf{letrec}}
\def \Case	{\Sf{case}}
\def \Of	{\Sf{of}}
\def \TGRS	{\Sc{tgrs}}
\def \ApTGRS	{\aps\Sc{tgrs}}
\def \CTRS	{\textsl {C\kern-3.8pt u\kern-1pt }\Sc{trs}}
%
% \def \ContSub#1[#2]{\setbox157=\hbox{$#2$}\ifdim\wd157<\One{\Rm {C}_{#1}}\else{\Rm {C}_{#1}\psk[\psk#2\psk]}\fi}
%\def \Contone[#1]{\@ifnextchar{\bgroup}{\Conttwo[#1]}{{\Rm {C}\psk[\psk#1\psk]}}}
\def \ContSub#1[#2]{\setbox157=\hbox{$#2$}\ifdim\wd157<\One{\Rm {C}_{#1}}\else{\Rm {C}_{#1}\psk[\psk#2\psk]}\fi}
\def \Contone[#1]{{\Rm {C}\psk[\psk#1\psk]}}
\def \Cont{\@ifnextchar[{\Contone}{\ContSub}}
%
\def \Contatwo[#1]#2{\setbox157=\hbox{$#2$}\ifdim\wd157<\One{\Rm {C}'_{#1}}\else{\Rm {C}'_{#1}\skp[\psk#2\psk]}\fi}
\def \Contaone[#1]{\@ifnextchar{\bgroup}{\Contatwo[#1]}{{\Rm {C}'\psk[\psk#1\psk]}}}
\def \Conta{\@ifnextchar[{\Contaone}{\Rm {C}'}}
%
\def \repl#1{#1\raise3pt\hbox{\scrm {R}}}
\def \R	{\Rm{R}}
\def \Rfn	{\scrm {R}}
%\def \redr {\rightarrow_{\mbox {\scbf {r}}}} 
%\def \red	{\rightarrow}
%\def \reds	{{\rightarrow}}
\def \redplus	{\mathrel{\arrow^+}}
%\def \dred	{\Skip\arrow^*\Skip}
%\def \reddR	{\dred}
\def \vars	{{\cal X}}
\def \Rules {\Bf {R}}

\def \Ax {\textsl {Ax}}
\def \arrI	{\arrow \textsl{I}}
\def \arrE	{\arrow \textsl{E}}
\def \intI	{\inter \textsl{I}}
\def \intE	{\inter \textsl{E}}
\def \quaI	{\forall \textsl{I}}
\def \quaE	{\forall \textsl{E}}

\def \TBs 	{\Tstrict{\langle `G,`s\rangle}}
\def \TBt 	{\Tstrict{\langle `G,`t\rangle}}
\def \EV	{{\cal V}_{`f}\langle `G,`s\rangle}
\def \LTv#1{\textsl{last-tv}\,(#1)}	

\def \Types	{{\cal T}}
\def \TBCD	{{\cal T}_{\BCDscript}}
\def \Tc	{\Types_{\scsc {c}}}
\def \Tone 	{\Types_{\kern-1pt\scit {1}}}
\def \Tqc	{\Types^\forall_{\scit {C}}}
\def \Tqone 	{\Types^\forall_{\kern-1pt\scit {1}}}
\def \Tqtwo 	{\Types^\forall_{\scit {2}}}
\def \Ttwo 	{\Types_{\scit {2}}}
\def \Tca	{\Types'_{\scit {C}}}
\def \Tstrict 	{\Types_{\scsc {s}}}
\def \TStrict 	{\Types}%{\Types_{\scit {S}}}
\def \Tsn	{\Types_{\noomega}}
\def \Tps 	{\Types_{\mbox{\scit s}}}
\def \TpS 	{\Types}

\def \lb {\lambda{\perp}}
\def \Lb {\Lambda{\perp}}
\def \bottom {{\perp}}
\def \con	{\mathbin{\ast}}
\def \after	{{\circ}\hspace*{0.5pt}}
\def \ele {\mathbin{\in}} 
\def \same	{\mathbin{\equiv}}
\def \equ	{\mathop{\sim}}
% \def \Stat#1#2{#1\skp{:}\skp#2}

\def \by {\mathop{\mapsto}}
\def \subs {(\tvar \by \rho)}
\def \stsub	{(\varphi \by `j)}
\def \subone#1{\stsub\,(#1)}
\def \sub	{\@ifnextchar{\bgroup}{\subone}{\stsub}}
\def \subst#1{(\varphi \by #1)}
\def \IdS	{\mbox	{$\textsl {Id}_S$}}
\def \Subst	{\mbox	{$\cal S$}}
\def \subs {(\varphi \by \rho)}
\def \Si#1{\textsl {S}_{#1}}
\def \Stwo#1#2{\setbox157=\hbox{$#2$}\ifdim\wd157<\One \Si{#1}\else\Si{#1}\skp({#2})\fi}
\def \Sone#1{\@ifnextchar{\bgroup}{\Stwo{#1}}{\textsl {S}\skp(#1)}}
\def \S{\@ifnextchar{\bgroup}{\Sone}{\textsl {S}}}
\def \Sub{\S}
\def \Sotn	{\S_1, \ldots, \S_n}
\def \Sotm	{\S_1, \ldots, \S_m}
\def \Satwo#1#2{\setbox157=\hbox{$#2$}\ifdim\wd157<\One{\textsl {S}'_{#1}}\else{\textsl {S}'_{#1}\skp(#2)}\fi}
\def \Saone#1{\@ifnextchar{\bgroup}{\Satwo{#1}}{\textsl {S}'\skp (#1)}}
\def \Sa{\@ifnextchar{\bgroup}{\Saone}{\textsl {S}'}}

\def \Etwo#1#2{\setbox157=\hbox{$#2$}\ifdim\wd157<\One{\textsl {Ex}_{#1}}\else{\textsl {Ex}_{#1}\skp(#2)}\fi}
\def \Eone#1{\@ifnextchar{\bgroup}{\Etwo{#1}}{\textsl {Ex}\skp(#1)}}
\def \E{\@ifnextchar{\bgroup}{\Eone}{\textsl {Ex}}}
\def \dunBs {n_\Pair{`G,\sigma}}
\def \Ev{\Vec{\textsl{Ex}}}
\def \Evi#1{\Ev_{#1}}

\def \Ltwo#1#2{\setbox157=\hbox{$#2$}\ifdim\wd157<\One{\textsl {L}_{#1}}\else{\textsl {L}_{#1}\skp(#2)}\fi}
\def \Lone#1{\@ifnextchar{\bgroup}{\Ltwo{#1}}{\textsl {L}\skp(#1)}}
\def \L{\@ifnextchar{\bgroup}{\Lone}{\textsl {L}}}
\def \La	{\L'}
%\def \Lifting#1#2{{<}\Pair{#1},\Pair{#2}{>}}
\def \Lifting#1#2{\Pair{\Pair{#1},\Pair{#2}}}

\def \Cl	{\textsl {Cl}}
\def \Clotn	{\Cl_1, \ldots, \Cl_n}
\def \Close#1{\mbox{${\langle #1 \rangle}$}}

\def \Covone#1{{\prec}#1{\succ}}
\def \Covi#1{\textsl {Cov}\,(#1)}
\def \Cov	{\@ifnextchar{\bgroup}{\Covone}{\textsl {Cov}}}

\def \O{\textsl {O}}
\def \Oi#1{\textsl {O}_{#1}}

\def \Chaintwo#1#2{[#1]\skp(#2)}
\def \Chain#1{\@ifnextchar{\bgroup}{\Chaintwo{#1}}{[#1]}}
\def \Chains	{\mbox	{${\cal C}$\textsl {h}}}
\def \Chitwo#1#2{\setbox157=\hbox{$#2$}\ifdim\wd157<\One{\textsl {Ch}_{#1}}\else{\textsl {Ch}_{#1}\skp(#2)}\fi}
\def \Chione#1{\@ifnextchar{\bgroup}{\Chitwo{#1}}{\textsl {Ch}\skp(#1)}}
\def \Ch{\@ifnextchar{\bgroup}{\Chione}{\textsl {Ch}}}
\def \Cha	{\Ch'}
\def \Chotn	{\Ch_1, \ldots, \Ch_n}
\def \Chotm	{\Ch_1, \ldots, \Ch_m}
\def \Cotimo	{\Ch_1, \ldots, \Ch_{i-1}}
\def \CF {\textsl {Ch}_F}

\def \tvar	{\varphi}
\def \observe{\item[]}

\def \append	{\Sf{append}}
\def \cons	{\Sf{cons}}
\def \nil	{\Sf{nil}}
\def \map	{\Sf{map}}
\def \maptwice	{\Sf{maptwice}}
\def \Succ	{\Sf{Succ}}
\def \Cons	{\Sf{cons}}
\def \List	{\Sf{list}}
\def \Nil	{\Sf{[]}}
%\def\proof{\Proof}
%\def\endproof{\endProof}

\def \List#1{[#1]}
\def \IsEmptyList	{\Sf{IsNil}}%{\underline{{=}\List{}}}
\def \Bool	{\Sf{Bool}}
\def \True	{\Sf{t\kern-1pt t}}
\def \False	{\Sf{f\kern-1pt f}}

%\def \FixML	{\Tt{F}\kern-.5pt\Tt{i}\kern-.5pt\Tt{x}}
\def \FixML	{\textsl{Fix}}

%AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
\def \longarrow#1{\psset{unit=1\point,linewidth=0.3\point}
\hspace*{.9#1}\pscurve{cc-cc}(0,1.5)(-1.1,2)(-2.25,3.5)\hspace*{.1#1}}

\newdimen\arrowlength
\def \longarrow#1{\psset{unit=1\point,linewidth=0.3\point}%
\arrowlength#1\advance\arrowlength-1\point
\psline{cc-cc}(1,1)(\arrowlength,1)%
\hspace*{\arrowlength}\pscurve{cc-cc}(0,1)(-1.1,1.5)(-2.25,2.5)\hspace*{1\point}}

\def \Vec#1{\setbox155=\hbox{$#1$}%
\leavevmode\copy155\kern-\wd155% put argument and move left
\raise\ht155\hbox{\longarrow{\wd155}}}

\newlength\harpoonlength
\def \longharpoon#1{\psset{unit=.7\point,linewidth=0.4\point}%
\harpoonlength#1\addtolength{\harpoonlength}{-1\point}%
\psline{cc-cc}(-1,1.5)(-\harpoonlength,1.5)%
\pscurve{cc-cc}(-0.7,1.5)(-1.5,1.69)(-2,2.05)(-2.5,2.55)(-3,3.35)
\vbox to 2\point{}%
}
\def \Vec#1{\setbox155=\hbox{$#1$}%
\leavevmode\copy155\raise\ht155\hbox{\longharpoon{\wd155}}}

\def\Overline#1{%
	\psset{unit=1\point,linewidth=0.35\point}
	\setbox155=\hbox{$#1$}\leavevmode
	\raise\ht155\hbox{\psline{c-c}(.05\wd155,1.25)(.95\wd155,1.25)}\box155% 
}
%
\def\underline#1{%
	\psset{unit=1\point,linewidth=0.45\point}
	\setbox156=\hbox{${#1}$}\leavevmode
	\raise-\dp156\hbox{\psline{c-c}(.05\wd156,-1.25)(.95\wd156,-1.25)}\box156%
}

\def \iotk	{i \ele \k}%{1{\,{\leq}\,} i{\,{\leq}\,}k}
\def \iotn	{i \ele \n}%{1{\,{\leq}\,} i{\,{\leq}\,}n}
\def \iotm	{i \ele \m}%{i \ele \k}%{1{\,{\leq}\,} i{\,{\leq}\,}m}
\def \jotm	{j \ele \m}%{1{\,{\leq}\,} j{\,{\leq}\,}m}
\def \jotn	{j \ele \n}%{1{\,{\leq}\,} j{\,{\leq}\,}n}
\def \jnotiotn	{1{\,{\leq}\,} j \not = i{\,{\leq}\,}n}
\def \iotnmo	{1{\,{\leq}\,} i{\,{\leq}\,}n{-}1}
\def \jotp	{j \ele \p}%{1{\,{\leq}\,} j{\,{\leq}\,}p}
\def \kotm	{k \ele \m}%{1{\,{\leq}\,} k{\,{\leq}\,}m}
\def \iotnfn	{1{\leq} i{\leq}n}
\def \jotmfn	{1{\leq} j{\leq}m}

\def \aoIm	{\alpha_1{\inter}{\dots}{\inter}\alpha_m}
\def \aotk		{\alpha_1, \ldots ,\alpha_k}
\def \aoIn	{\alpha_1{\copy149}{\dots}{\copy149}\alpha_n}
\def \soIn	{\sigma_1{\copy149}{\dots}{\copy149}\sigma_n}
\def \soIna	{\sigma'_1{\copy149}{\dots}{\copy149}\sigma'_n}
\def \soIm	{\sigma_1{\copy149}{\dots}{\copy149}\sigma_m}
\def \soIma	{\sigma'_1{\copy149}{\dots}{\copy149}\sigma'_m}
\def \gAd {\gamma\arrow\delta}
\def \goAgnAg {\gamma_1{\arrow}{\dots}{\arrow}\gamma_n{\arrow} \gamma}
\def \gotn		{\gamma_1, \ldots ,\gamma_n}
\def \moIn	{\mu_1{\inter}{\dots}{\inter}\mu_n}
\def \poIn	{\pi_1{\inter}{\dots}{\inter}\pi_n}
\def \rAm	{\rho\arrow\mu}
\def \roIn	{\rho_1{\inter}{\dots}{\inter}\rho_n}
\def \sAt	{\sigma\arrow\tau}
\def \sIt	{\sigma \inter \tau}
\def \soAsnAs {\sigma_1{\arrow}{\dots}{\arrow}\sigma_n{\arrow} \sigma}
\def \soaAsnaAsa {\sigma'_1{\arrow}{\dots}{\arrow}\sigma'_n{\arrow} \sigma'}
\def \soaAsnaAs {\sigma'_1{\arrow}{\dots}{\arrow}\sigma'_n{\arrow} \sigma}
\def \soAsnAt {\sigma_1{\arrow}{\dots}{\arrow}\sigma_n{\arrow} \tau}
\def \tAs	{\tau\arrow\sigma}
\def \rAr	{\rho\arrow\rho}
\def \wAr	{\omega\arrow\rho}
\def \tAr	{\tau\arrow\rho}
\def \toIn	{\tau_1{\inter}{\dots}{\inter}\tau_n}
\def \toIm	{\tau_1{\inter}{\dots}{\inter}\tau_m}
\def \toIna	{\tau'_1{\copy149}{\dots}{\copy149}\tau'_n}
\def \wAs	{\omega\arrow\sigma}
\def \wAt	{\omega\arrow\tau}
\def \wAwAf	{\omega\arrow \dots \arrow \omega \arrow \tvar}

\def \FVar {\Phi}
\def \BVar {{\cal A}}

\def \Envone#1{{\cal E}\skp(#1)}
\def \Env{\@ifnextchar{\bgroup}{\Envone}{{\cal E}}}
%\def \EnvCLone#1{{\cal E}_{\scsc {cl}}\skp(#1)}
%\def \EnvCL{\@ifnextchar{\bgroup}{\EnvCLone}{{\cal E}_{\mbox{\scsc {cl}}}}}
\def \EnvCL {\Env}
\def \Pair#1{{\langle#1\rangle}}
\def \last#1{\textsl{last}\skp(#1)}
\def \ExmnBs#1{\langle `f, n, `G, `s \rangle\,(#1)}
\def \exmnBs	{\langle `f, n, `G, `s \rangle}
\def \sotn	{\sigma_1, \ldots, \sigma_n}
\def \sotm	{\sigma_1, \ldots, \sigma_m}
\def \totn	{\tau_1, \ldots, \tau_n}
\def \totm	{\tau_1, \ldots, \tau_m}
\def \union	{{\,\cup\,}}
\def \Except	{{\setminus}}
\def \toIn	{\tau_1{\copy149}{\dots}{\copy149}\tau_n}
\def \toIm	{\tau_1{\copy149}{\dots}{\copy149}\tau_m}
\def \Bases	{{\cal B}}
\def \prB#1{\ifnextchar{\bgroup}{\prBtwo{#1}}{\mbox{\large $\cap$}\{#1\}}}
\def \prBtwo#1#2{\mbox{\large $\cap$}_{#1}#2}
\def \Botn	{B_1, \ldots, B_n}
\def \PoPn	{P_1, \ldots, P_n}

\newcommand{\mathsmall}[1]{\mbox{\small$#1$}}

\def\smallerfont{\fontsize{\@ixpt}{10.8pt}\selectfont}
\def\tinyfont{\fontsize{12pt}{14pt}\selectfont}

\def\DerRule(#1){(#1)}

\def \intsymb	{\mbox {\small {$\cap$}}}%{\mbox {\small {$\wedge$}}}%
\def \intTwo#1(#2){\intsymb_{#1}(#2)}
\def \intOne#1{\@ifnextchar({\intTwo{#1}}{\intsymb_{#1}}}
\def \int{\@ifnextchar\bgroup{\intOne}{\intsymb}}

\def\G_#1{`G\kern-1pt_{#1}}
\def \GamoU#1{\un{#1}\G_i}
\def \GamoI#1{{\int{#1}\G_i}}
\def \Gamot#1{\G_i\,(i \ele #1)}

\def \HNF{{\cal H}}
\def \HN{{\cal H}}
\def \ggtNF{\mathrel{>>_{\cal NF}}}
\def \Signature	{({\cal F}\kern-.3em, {\cal X})}
\def \OrderNF   {(\smallerN, \Encom, \succ)_{\Em {lex}}}


